Gradient Tracking for High Dimensional Federated Optimization

In this paper, we study the (decentralized) distributed optimization problem with high-dimensional sparse structure. Building upon the FedDA algorithm, we propose a (Decentralized) FedDA-GT algorithm, which combines the \textbf{gradient tracking} technique. It is able to eliminate the heterogeneity among different clients' objective functions while ensuring a dimension-free convergence rate. Compared to the vanilla FedDA approach, (D)FedDA-GT can significantly reduce the communication complexity, from ${O}(s^2\log d/\varepsilon^{3/2})$ to a more efficient ${O}(s^2\log d/\varepsilon)$. In cases where strong convexity is applicable, we introduce a multistep mechanism resulting in the Multistep ReFedDA-GT algorithm, a minor modified version of FedDA-GT. This approach achieves an impressive communication complexity of ${O}\left(s\log d \log \frac{1}{\varepsilon}\right)$ through repeated calls to the ReFedDA-GT algorithm. Finally, we conduct numerical experiments, illustrating that our proposed algorithms enjoy the dual advantage of being dimension-free and heterogeneity-free.

==> Algorithms/decentral_fedda.tex <==
\begin{algorithm}
  \caption{\dfeddualavgfull (\dfeddualavg)}
  \label{alg:dfeddualavg}
  \begin{algorithmic}[1]
  \STATE {\textbf{procedure}} \dfeddualavg ($w_0, \eta_{\client}, \eta_{\server}$)
  \STATE $z_{0} \gets \nabla h(w_0)$ \COMMENT{server dual initialization}
  \FOR {$r=0, \ldots, R-1$}
    \STATE sample a random gossip matrix $\rmU^{(r)} \sim \gU$
      \FORALL {\kern-6.5em\tikzmark{dfeddualavg:begin}\kern+6.5em $m \in [M]]$ {\bf in parallel}}
        \FOR {$k = 0, \ldots, K-1$}
          % \STATE $\tilde{\eta}_{r,k} \gets \eta_{\server} \eta_{\client} r K + \eta_{\client} k$ 
          \STATE $\vw_{r,k}^m \gets \nabla^{-1}h(\vz_{r,k}^m)$
            \COMMENT{retrieve primal}
          \STATE $\vg_{r,k}^m \gets \nabla F (\vw_{r,k}^m; \xi_{r,k}^m) $
            \COMMENT{query gradient}
          \STATE $\vz_{r,k+1}^m \gets \vz_{r,k}^m - \eta_{\client} \vg_{r,k}^m$
            \COMMENT{client \emph{dual} update\tikzmark{dfeddualavg:end}}
          % \STATE \COMMENT{client update\tikzmark{fedmid:end}} 
          \drawCodeBox{fill=purple}{dfeddualavg:begin}{dfeddualavg:end}
        \ENDFOR
      \STATE $\Delta_r^m = \ssum{l}{1}{M}u^{(r)}_{lm}(\vz_{r,K}^l - \vz_{r,0}^l)$
        \COMMENT{decentralized communication}
      \STATE $\vz_{r+1,0}^m = \vz_{r,0} + \eta_{\server}\Delta_r^m$
        \COMMENT{next round \emph{dual} update}
      \ENDFOR
  \ENDFOR
\end{algorithmic}
\end{algorithm}

==> Algorithms/feddual_alg.tex <==
% !TEX root = main.tex  
\begin{algorithm}
  \caption{\feddualavgfull (\feddualavg)}
  \label{alg:feddualavg}
  \begin{algorithmic}[1]
  \STATE {\textbf{procedure}} \feddualavg ($w_0, \eta_{\client}, \eta_{\server}$)
  \STATE $\vz_{0} \gets \nabla h(\vw_0)$ \COMMENT{server dual initialization}
  \FOR {$r=0, \ldots, R-1$}
    \STATE sample a subset of clients $\mathcal{S}_r \subseteq [M]$
      \FORALL {\kern-6.5em\tikzmark{feddualavg:begin}\kern+6.5em $m \in \mathcal{S}_r$ {\bf in parallel}}
        \STATE $\vz_{r,0}^m \gets \vz_{r}$ \COMMENT{broadcast \emph{dual} initialization}
        \FOR {$k = 0, \ldots, K-1$}
          % \STATE $\tilde{\eta}_{r,k} \gets \eta_{\server} \eta_{\client} r K + \eta_{\client} k$ 
          \STATE $\vw_{r,k}^m \gets \nabla^{-1}h(\vz_{r,k}^m)$
            \COMMENT{retrieve primal}
          \STATE $\vg_{r,k}^m \gets \nabla F (\vw_{r,k}^m; \xi_{r,k}^m) $
            \COMMENT{query gradient}
          \STATE $\vz_{r,k+1}^m \gets \vz_{r,k}^m - \eta_{\client} \vg_{r,k}^m$
            \COMMENT{client \emph{dual} update\tikzmark{feddualavg:end}}
          % \STATE \COMMENT{client update\tikzmark{fedmid:end}} 
          \drawCodeBox{fill=blue}{feddualavg:begin}{feddualavg:end}
        \ENDFOR
      \ENDFOR
  \STATE $\Delta_r = \frac{1}{|\mathcal{S}_r|} \sum_{m \in \mathcal{S}_r} (\vz_{r, K}^m - \vz_{r, 0}^m)$
  \STATE $\vz_{r+1} \gets \vz_{r} + \eta_{\server} \Delta_r$
            \COMMENT{server \emph{dual} update}
  \STATE $\vw_{r+1} \gets \nabla^{-1} h  (\vz_{r+1})$
            \COMMENT{(optional) retrieve server primal state}
  \ENDFOR
\end{algorithmic}
\end{algorithm}


==> Algorithms/multi_redfedda_alg.tex <==
\begin{algorithm}
  \caption{\multiredfeddafull (\multiredfedda)}
  \label{alg:multiredfedda}
  \begin{algorithmic}[1]
  \STATE {\textbf{procedure}} \multiredfedda ($w_0^m, \eta_{\client}, \eta_{\server}$, Q_0, R_n,K_n, N)
  \FOR{n= 0, \ldots, N}
\end{algorithmic}
\end{algorithm}

==> Algorithms/restricted_decentral_fedda_alg.tex <==
\begin{algorithm}
  \caption{\redfeddafull (\redfedda)}
  \label{alg:redfedda}
  \begin{algorithmic}[1]
  \STATE {\textbf{procedure}} \redfedda ($w_0^m, \eta_{\client}, \eta_{\server}, Q, R, E$)
  \STATE $z_{0} \gets \nabla h(0)$ \COMMENT{server dual initialization}
  \FOR {$r=0, \ldots, R-1$}
    \STATE sample a random gossip matrix $\rmU^{(r)} \sim \gU$
      \FORALL {\kern-6.5em\tikzmark{redfedda:begin}\kern+6.5em $m \in [M]]$ {\bf in parallel}}
        \FOR {$k = 0, \ldots, K-1$}
          % \STATE $\tilde{\eta}_{r,k} \gets \eta_{\server} \eta_{\client} r K + \eta_{\client} k$ 
          \STATE $\vg_{r,k}^m \gets \nabla F (\vw_{r,k}^m; \xi_{r,k}^m) $
            \COMMENT{query gradient}
          \STATE $\vz_{r,k+1}^m \gets \vz_{r,k}^m - \eta_{\client} \vg_{r,k}^m$
            \COMMENT{client \emph{dual} update\tikzmark{redfedda:end}}
          \STATE $\vw_{r,k}^m \gets \nabla^{-1}h(\vz_{r,k}^m) + \vw_{0}$
            \COMMENT{retrieve primal}
          % \STATE \COMMENT{client update\tikzmark{fedmid:end}} 
          \drawCodeBox{fill=purple}{redfedda:begin}{redfedda:end}
        \ENDFOR
      \STATE $\Delta_r^m = \ssum{l}{1}{M}u^{(r)}_{lm}(\vz_{r,K}^l - \vz_{r,0}^l)$
        \COMMENT{decentralized communication}
      \STATE $\vz_{r+1,0}^m \gets \vz_{r,0} + \eta_{\server}\Delta_r^m$
        \COMMENT{next round \emph{dual} update}
      \STATE $\vw_{r+1,0}^m \gets \argmin\limits_{\norm{\vw - \vw_0^m}_q \le Q} \left\{
      \inner{\vw - \vw_0}{\vz_{r+1,0}^m} + h(\vw - \vw_0)
      \right\}$  
        \COMMENT{project back into the feasible set}
      \ENDFOR
  \ENDFOR
  \STATE $\hat{\vw}^m \gets \textsc{Sparse}\left( \frac{1}{R}\ssum{r}{0}{R-1} \vw_{r,0}^m \right)$
\end{algorithmic}
\end{algorithm}

==> Algorithms/scaffoldDA_alg.tex <==
% !TEX root = main.tex  
\begin{algorithm}
  \caption{\scaffolddafull  (\scaffoldda)}
  \label{alg:scaffoldda}
  \begin{algorithmic}[1]
  \STATE {\textbf{procedure}} \feddualavg ($\vw_0, \eta_{\client}, \eta_{\server}$)
  \STATE $\vz_{0} \gets \nabla h(\vw_0)$ \COMMENT{server dual initialization}
  \FOR {$r=0, \ldots, R-1$}
    \STATE sample a subset of clients $\mathcal{S}_r \subseteq [M]$
      \FORALL {\kern-6.5em\tikzmark{scaffoldda1:begin}\kern+6.5em $m \in \mathcal{S}_r$ {\bf in parallel}}
        \STATE $\vz_{r,0}^m \gets \vz_{r}$ \COMMENT{broadcast \emph{dual} initialization}
        \FOR {$k = 0, \ldots, K-1$}
          % \STATE $\tilde{\eta}_{r,k} \gets \eta_{\server} \eta_{\client} r K + \eta_{\client} k$ 
          \STATE $\vw_{r,k}^m \gets \nabla^{-1}h(\vz_{r,k}^m)$
            \COMMENT{retrieve primal}
          \STATE $\vg_{r,k}^m \gets \nabla F (\vw_{r,k}^m; \xi_{r,k}^m) - \vc_r^m + \vc_r $
            \COMMENT{query gradient with controller calibration}
          \STATE $\vz_{r,k+1}^m \gets \vz_{r,k}^m - \eta_{\client} \vg_{r,k}^m$
            \COMMENT{client \emph{dual} update\tikzmark{scaffoldda1:end}}
          % \STATE \COMMENT{client update\tikzmark{fedmid:end}} 
          \drawCodeBox{fill=blue}{scaffoldda1:begin}{scaffoldda1:end}
        \ENDFOR
      \ENDFOR
  \STATE \tikzmark{scaffoldda2:begin} $\vc_{r+1}^m \gets \vc_{r}^m - \vc_r - \frac{1}{K\eta_c}(\vz_{r,K}^m - \vz_{r,0}^m)$
    \COMMENT{maintain controller}
  \STATE $\vc_{r+1} = \vc_r + \frac{1}{M}\sum\limits_{m\in \gS_r}(\vc_{r+1}^m - \vc_r^m)$
  \STATE $\Delta_r = \frac{1}{|\mathcal{S}_r|} \sum_{m \in \mathcal{S}_r} \vc_{r+1}^m$
    \COMMENT{aggregate gradient information\tikzmark{scaffoldda2:end}}
  \drawCodeBox{fill=orange}{scaffoldda2:begin}{scaffoldda2:end}
  \STATE $\vz_{r+1} \gets \vz_{r} + K\eta_{\server} \Delta_r$
            \COMMENT{server \emph{dual} update}
  \STATE $\vw_{r+1} \gets \nabla^{-1} h  (\vz_{r+1})$
            \COMMENT{(optional) retrieve server primal state}
  \ENDFOR
\end{algorithmic}
\end{algorithm}


==> Proofs/proof_for_central_conv.tex <==
\begin{lemma}[One-step analysis]\label{lem:1_step_fedda}
Let Assumptions~\ref{asp:convex} - \ref{asp:grad_subG} hold. Then there is a universal constant $C$ such that for the sequences $\{\vw_{r+1,k}\}, \{\vz_{r+1,k}\}$ generated from both Algorithm~\ref{alg:feddualavg} and Algorithm~\ref{alg:scaffoldda}, we have
\begin{align*}
&\EB\rmD_h(\vw^*, \vw_{r+1,0}) - \EB\rmD_h(\vw^*, \vw_{r,0}) \le
-\EB\rmD_h (\vw_{r+1,0}, \vw_{r,0}) + \frac{2Cp^4d^{2/p}K\sigma^2 \eta^2}{M}\\
 &+ \left(\frac{Ld^{2/p} \eta}{2M} + \frac{8d^{4/p} KL^2 \eta^2}{M}\right)\ssum{m}{1}{M}\ssum{k}{0}{K-1} \EB \norm{\vz_{r,k}^m - \vz_{r,0}}_p^2 + (K\eta - 8d^{2/p}\eta^2 K^2 L) \EB\left\{f(\vw^*) - f(\vw_{r,0})\right\}.
\end{align*}
\end{lemma}

\begin{lemma}[One-step deviation of FedDA]\label{lem:local_dev_fedda}
Under the assumptions of Theorem~\ref{thm:conv_rt_fedda}, for any $k = 0,\cdots , K-1; ~ m \in [M]$, it is true that
\begin{align*}
\EB \norm{\vz_{r,k}^m - \vz_{r,0}}_p^2 \le 3d^{4/p}L^2 k\eta^2 \ssum{i}{0}{k-1}\EB \norm{\vz_{r,i}^m - \vz_{r,0}}_p^2 + 3Cd^{2/p}p^4 \sigma^2 k \eta^2 + 3k^2 \eta^2 \gD_r^m,
\end{align*}
with
\begin{align*}
\gD_r^m := 2\norm{\nabla f_m(\vw^*)}_p^2 + 4d^{2/p}L\EB \left\{
f_m(\vw_{r,0}) - f_m(\vw^*) - \inner{\nabla f_m(\vw^*)}{\vw_{r,0} - \vw^*}
\right\}.
\end{align*}
\end{lemma}



\begin{lemma}[One-step deviation of ScaffoldDA]\label{lem:local_dev_scaffoldda}
For simplicity we denote $\ssum{k}{0}{K-1}\ssum{m}{1}{M}\EB \norm{\vz_{r,k}^m - \vz_{r,0}}_p^2$ as $\gE_r$. Under the assumptions of Theorem~\ref{thm:conv_rt_scaffoldda}, for any $r = 1, \cdots, R; ~ k=0,\cdots, K-1; ~ m \in [M]$, we can derive that
\begin{align*}
\gE_r &\le 72 d^{4/p}L^2K^2\eta^2 \gE_{r-1} + Cd^{2/p}p^4\sigma^2MK^2\eta^2\\
&+ 54 MK^3\eta^2 \EB \norm{\nabla f(\vw_{r-1,0})}_p^2 + 18d^{4/p}L^2MK^3\eta^2 \EB \norm{\vw_{r,0} - \vw_{r-1,0}}_q^2.
\end{align*}
\end{lemma}

\begin{proof}[Proof of Theorem~\ref{thm:conv_rt_fedda}]
From Lemma~\ref{lem:local_dev_fedda},
\begin{align*}
&\ssum{i}{0}{k}\EB \norm{\vz_{r,i}^m - \vz_{r,0}}_p^2 = \ssum{i}{0}{k-1}\EB \norm{\vz_{r,i}^m - \vz_{r,0}}_p^2 + \EB \norm{\vz_{r,k}^m - \vz_{r,0}}_p^2\\
&\le \left( 1 + 3d^{4/p}L^2 k \eta^2 \right) \left( \ssum{i}{0}{k-1} \EB \norm{\vz_{r,i}^m - \vz_{r,0}}_p^2\right) + 3Cd^{2/p}p^4 \sigma^2 k \eta^2 + 3k^2 \eta^2 \gD_{r}^m\\
&\le \left( 1 + 3d^{4/p}L^2 k \eta^2 \right) \left( \ssum{i}{0}{k-1} \EB \norm{\vz_{r,i}^m - \vz_{r,0}}_p^2\right) + \left(3Cd^{2/p}p^4 \sigma^2 K \eta^2 + 3K^2\eta^2 \gD_r^m \right).
\end{align*}
Let $a = 3d^{4/p}L^2$, $b = 3Cd^{2/p}p^4 \sigma^2 K \eta^2 + 3K^2\eta^2 \gD_r^m$ and $\vs_k = \ssum{i}{0}{k}\EB \norm{\vz_{r,i}^m - \vz_{r,0}}_p^2$. According to Lemma~\ref{lem:rcs_to_etr_fedda}, let $\eta \le \frac{1}{2d^{2/p}LK}$, then
\begin{align*}
\ssum{k}{0}{K-1}\EB \norm{\vz_{r,i}^m - \vz_{r,0}}_p^2 \le 9Cd^{2/p}p^4\sigma^2 K^2 \eta^2 + 9K^3\eta^2 \gD_r^m.
\end{align*}
Furthermore,
\begin{equation}\label{eq:lcl_dev_fedda}
\begin{aligned}
&\ssum{m}{1}{M}\ssum{k}{0}{K-1}\EB \norm{\vz_{r,i}^m - \vz_{r,0}}_p^2 \le 9Cd^{2/p}p^4\sigma^2 M K^2 \eta^2
+ 9K^3\eta^2 \ssum{m}{1}{M}\gD_{r}^m\\
&= 9Cd^{2/p}p^4\sigma^2MK^2\eta^2 + 18 K^3\eta^2 \ssum{m}{1}{M}\norm{\nabla f_m(\vw^*)}_p^2\\
&+ 36 d^{2/p} LK^3\eta^2 \ssum{m}{1}{M}\left\{ f_m(\vw_{r,0}) - f_m(\vw^*) - \inner{\nabla f_m(\vw^*)}{\vw_{r,0} - \vw^*} \right\}\\
&= 9 Cd^{2/p}p^4\sigma^2MK^2\eta^2 + 18 K^3\eta^2 \ssum{m}{1}{M}\norm{\nabla f_m(\vw^*)}_p^2\\
&+ 36 d^{2/p}MLK^3\eta^2 \left\{f(\vw_{r,0}) - f(\vw^*) + \inner{\nabla f(\vw^*)}{\vw_{r,0} - \vw^*}\right\}\\
&\overset{(a)}{=} 9 Cd^{2/p}p^4\sigma^2MK^2 \eta^2 + 36 d^{2/p}MLK^3\eta^2 \EB\left\{f(\vw_{r,0}) - f(\vw^*)\right\} + 18 K^3\eta^2 \ssum{m}{1}{M}\norm{\nabla f_m(\vw^*)}_p^2.
\end{aligned}
\end{equation}
Here $(a)$ holds by the first order condition of the optimizer $\vw^*$. Letting $p = 2\log d$ and
plugging this bound and the magnitude constraint of $\eta$ into Lemma~\ref{lem:1_step_fedda} yield

\begin{equation}\label{eq:1_step_fedda_ut}
\begin{aligned}
&\EB\rmD_h(\vw^*, \vw_{r+1,0}) - \EB \rmD_h(\vw^*, \vw_{r,0})\le
-\EB \rmD_h(\vw_{r+1,0}, \vw_{r,0}) + \frac{96C(\log d)^4 \sigma^2 K\eta^2}{M} \\
&+ \frac{3L\eta}{M}\left\{
432 C (\log d)^4 \sigma^2 MK^2\eta^2 + 108 MLK^3\eta^2 \EB[f(\vw_{r,0}) - f(\vw^*)] 
\right\}
+ \frac{K\eta}{2}\EB [f(\vw^*) - f(\vw_{r,0})]\\
&+ \frac{3L\eta}{M}\cdot 18 K^3\eta^2 \ssum{m}{1}{M}\norm{\nabla f_m(\vw^*)}_p^2\\
&\le -\EB \rmD_h(\vw_{r+1,0}, \vw_{r,0}) + \frac{K\eta}{4} \EB [f(\vw^*) - f(\vw_{r,0})]
+ C(\log d)^4 \sigma^2 K\eta^2 (M^{-1} + LK\eta)\\
&+ \frac{54 L K^3\eta^3}{M} \ssum{m}{1}{M}\norm{\nabla f_m(\vw^*)}_p^2. 
\end{aligned}
\end{equation}
Summing \eqref{eq:1_step_fedda_ut} up, we get
\begin{align*}
\frac{K\eta}{4}\ssum{r}{0}{R-1} \EB [f(\vw_{r,0}) - f(\vw^*)] &\le \EB\rmD_h(\vw^*, \vw_{0,0})
+ C(\log d)^4 \sigma^2 RK\eta^2 (M^{-1} + LK\eta)\\
&+ \frac{54 LRK^3\eta^3}{M}\ssum{m}{1}{M}\norm{\nabla f_m(\vw^*)}_p^2.
\end{align*}
Recall the definition of $\hat{\vw}$ and combine it with the convexity of $f$, 
\begin{align*}
\EB f(\hat{\vw}) - f(\vw^*) &\le \frac{4\rmD_h(\vw^*,\vw_0)}{RK\eta} +
4C(\log d)^4 \sigma^2(M^{-1} + LK\eta)\eta 
+ \frac{216 LK^2\eta^2}{M}\ssum{m}{1}{M}\norm{\nabla f_m(\vw^\star)}_p^2 \\
&\lesssim \frac{\rmD_h(\vw^*,\vw_0)}{RK\eta} +
(\log d)^4 \sigma^2\eta 
+ LK^2 \gE_M^* \eta^2,
\end{align*}
where $\gE_M^* := \frac{1}{M}\ssum{m}{1}{M}\norm{\nabla f_m(\vw^\star)}_p^2$.

Finally, we optimize over the scale of the step size $\eta$. Recall that $\eta\leq \frac{1}{48LK}$. If $\frac{1}{48LK} \leq  \frac{\rmD_h(\vw^*,\vw_0)^{1/3}}{(LR\gE_M^*)^{1/3}K}$ and $\frac{1}{48LK} \leq \frac{\rmD_h(\vw^*,\vw_0)^{1/2}}{(RK)^{1/2}(\log d)^2 \sigma}$, then we choose $\eta=\frac{1}{48LK}$ to get
\begin{align*}
    \EB f(\hat{\vw}) - f(\vw^*) &\lesssim \frac{\rmD_h(\vw^*,\vw_0)LK}{RK} + LK^2\gE_M^*\cdot \left[\frac{\rmD_h(\vw^*,\vw_0)^{1/3}}{(LR\gE_M^*)^{1/3}K}\right]^2 + (\log d)^4 \sigma^2 \cdot \left[\frac{\rmD_h(\vw^*,\vw_0)^{1/2}}{(RK)^{1/2}(\log d)^2 \sigma}\right] \\
    &\lesssim \frac{\rmD_h(\vw^*,\vw_0)L}{R} + \frac{\rmD_h(\vw^*,\vw_0)^{2/3}(L\gE_{M}^*)^{1/3}}{R^{2/3}} + \frac{\rmD_h(\vw^*,\vw_0)^{1/2}(\log d)^2 \sigma}{(RK)^{1/2}}.
\end{align*}
Otherwise, we choose $\eta=\min\left\{ \frac{\rmD_h(\vw^*,\vw_0)^{1/3}}{(LR\gE_M^*)^{1/3}K}, \frac{\rmD_h(\vw^*,\vw_0)^{1/2}}{(RK)^{1/2}(\log d)^2 \sigma} \right\}$ to get
\begin{align*}
    \EB f(\hat{\vw}) - f(\vw^*) &\lesssim \max\left\{ \frac{\rmD_h(\vw^*,\vw_0)^{2/3}(L\gE_{M}^*)^{1/3}}{R^{2/3}} + (\log d)^4 \sigma^2 \eta, \frac{\rmD_h(\vw^*,\vw_0)^{1/2}(\log d)^2 \sigma}{(RK)^{1/2}} + LK^2\gE_M^* \eta^2 \right\} \\
    &\lesssim \frac{\rmD_h(\vw^*,\vw_0)^{2/3}(L\gE_{M}^*)^{1/3}}{R^{2/3}} + \frac{\rmD_h(\vw^*,\vw_0)^{1/2}(\log d)^2 \sigma}{(RK)^{1/2}}.
\end{align*}
Combining the above two inequalities concludes the proof.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:conv_rt_scaffoldda}]
Consider the Lyapunov function $\gG_r := \EB \rmD_h(\vw^*, \vw_{r,0}) + \frac{L^2K\eta^2}{M} \gE_{r-1} + 126 d^{6/p}L^3K^3\eta^3 \EB \norm{\vw_{r,0} - \vw_{r-1,0}}_q^2$. First, combining Lemma~\ref{lem:1_step_fedda} and Lemma~\ref{lem:local_dev_scaffoldda}, we can obtain the following recursive inequality,
\begin{equation}\label{eq:1_step_scaffoldda}
\begin{aligned}
    &\left\{\EB \rmD_h(\vw^*, \vw_{r+1,0}) + \frac{L^2K\eta^2}{M} \gE_{r}\right\} -
    \left\{\EB \rmD_h(\vw^*, \vw_{r,0}) + \frac{L^2K\eta^2}{M} \gE_{r-1}\right\}\\
    \le&
    -\EB \rmD_h(\vw_{r+1,0}, \vw_{r,0}) + \frac{2Cp^4d^{2/p}K\sigma^2 \eta^2}{M} + \left( \frac{d^{2/p}L\eta}{2M} + \frac{8d^{4/p}L^2K\eta^2}{M} \right)\gE_r\\
    &+ (K\eta - 8d^{2/p}LK^2\eta^2)\EB \left\{ f(\vw^*) - f(
    \vw_{r,0}
    ) \right\} + \frac{L^2K\eta^2}{M} \gE_r - \frac{L^2K\eta^2}{M} \gE_{r-1}\\
    \le&
    -\EB \rmD_h(\vw_{r+1,0}, \vw_{r,0}) + \frac{2Cp^4d^{2/p}K\sigma^2 \eta^2}{M} + \frac{d^{2/p}L\eta}{M}\gE_r - \frac{L^2K\eta^2}{M}\gE_{r-1}\\
    &+
    \frac{K\eta}{2}\EB \left\{ f(\vw^*) - f(\vw_{r,0}) \right\}\\
    \le&
    -\EB \rmD_h(\vw_{r+1,0}, \vw_{r,0}) + \frac{2Cp^4d^{2/p}K\sigma^2 \eta^2}{M} + (72 d^{6/p}LK\eta - 1)\cdot \frac{L^2K\eta^2}{M} \gE_{r-1}\\
    &+ Cd^{4/p}p^4 \sigma^2 L K^2 \eta^3 + 54 d^{2/p}LK^3\eta^3 \EB \norm{\nabla f(\vw_{r-1,0})}_p^2\\
    &+ 18d^{6/p}L^3K^3\eta^3 \EB \norm{\vw_{r,0} - \vw_{r-1,0}}_q^2
    + \frac{K\eta}{2}\EB \left\{ f(\vw^*) - f(\vw_{r,0}) \right\}.
\end{aligned}
\end{equation}

Note that by the strong convexity of $h$, we have $\EB \norm{\vw_{r+1,0} - \vw_{r,0}}_q^2 \le 2\EB \rmD_h(\vw_{r+1,0}, \vw_{r,0})$. Furthermore, by making use of Lemma~\ref{lem:conj_sc}, we can derive
\begin{align*}
&\EB \norm{\nabla f(\vw_{r-1,0})}_p^2 = \EB \norm{\nabla f(\vw_{r-1,0}) - \nabla f(\vw^*)}_p^2\\
\le&
2\EB \norm{\nabla f(\vw_{r-1,0}) - \nabla f(\vw_{r,0})}_p^2 + 2\EB \norm{\nabla f(\vw_{r,0}) - \nabla f(\vw^*)}_p^2\\
\le&
2d^{4/p}L^2\EB \norm{\vw_{r-1,0} - \vw_{r,0}}_q^2 + 4d^{2/p}L\EB \left\{ f(\vw_{r,0}) - f(\vw^*) \right\}.
\end{align*}
Integrating these with \eqref{eq:1_step_scaffoldda} and using $32d^{2/p}LK\eta \le 1$ result in
\begin{align*}
    &\gG_{r+1} - \gG_{r}
    \le
    - (1 - 252d^{6/p}L^3K^3\eta^3)\rmD_h(\vw_{r+1,0}, \vw_{r,0}) + \left(\frac{1}{M} + d^{2/p}LK\eta \right)Cp^4d^{2/p}\sigma^2 K\eta^2\\
    &+ \left( \frac{K\eta}{2} - 216 d^{4/d}L^2K^3\eta^3 \right)\EB \left\{ f(\vw^*) - f(\vw_{r,0}) \right\}\\
    &\le \left(\frac{1}{M} + d^{2/p}LK\eta \right)Cp^4d^{2/p}\sigma^2 K\eta^2 + \frac{K\eta}{4}
    \EB \left\{ f(\vw^*) - f(\vw_{r,0}) \right\}.
\end{align*}
By telescoping we can get
\begin{align*}
    \frac{K\eta}{4}\EB \ssum{r}{0}{R-1}\left\{ f(\vw_{r,0}) - f(\vw^*) \right\}
    \le \gG_0 + \left( \frac{1}{M} + d^{2/p}LK\eta \right)Cp^4d^{2/p}\sigma^2 K\eta^2 R
\end{align*}
From Assumption~\ref{asp:convex} and the definition of $\Tilde{\vw}$, we finally get
\begin{align*}
    \EB f(\Tilde{\vw}) - f(\vw^*) \le \frac{4\gG_0}{RK\eta} + \left( \frac{1}{M} + d^{2/p}LK\eta \right) Cp^4d^{2/p}\sigma^2 \eta.
\end{align*}
Choosing $\eta = \min\left\{ \frac{1}{96LK}, \frac{\rmD_h(\vw^*,\vw_0)^{1/2}}{(RK)^{1/2}(\log d)^2 \sigma} \right\}$ concludes the proof.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:1_step_fedda}]
By the definition of Bregman divergence $\rmD_h$ and the fact that $\vz_{r,0}=\nabla h(\vw_{r,0})$, we can derive
\begin{equation}\label{eq:1_step_fedda_1}
\begin{aligned}
&\rmD_h(\vw^*,\vw_{r+1,0}) - \rmD_h(\vw^*, \vw_{r,0})\\
=& \left\{h(\vw^*) - h(\vw_{r+1,0}) - \inner{\vz_{r+1,0}}{\vw^* - \vw_{r+1,0}} \right\} - \left\{ h(\vw^*) - h(\vw_{r,0}) - \inner{\vz_{r,0}}{\vw^* - \vw_{r,0}} \right\}\\
=& -\left\{ h(\vw_{r+1,0}) - h(\vw_{r,0}) - \inner{\vz_{r,0}}{\vw_{r+1,0} - \vw_{r,0}} \right\} + \inner{\vz_{r,0} - \vz_{r+1,0}}{\vw^* - \vw_{r+1,0}}\\
=& - \rmD_h(\vw_{r+1,0}, \vw_{r,0}) + \inner{\vz_{r,0} - \vz_{r+1,0}}{\vw^* - \vw_{r,0}} + \inner{\vz_{r+1,0} - \vz_{r,0}}{\vw_{r+1,0} - \vw_{r,0}}.
\end{aligned}
\end{equation}

Next, we will bound the last two terms respectively. Note for both Algorithm~\ref{alg:feddualavg} and Algorithm~\ref{alg:scaffoldda}, it always holds that $\vz_{r,0} - \vz_{r+1,0} = \frac{\eta}{M}\ssum{m}{1}{M}\ssum{k}{0}{K-1}\nabla F(\vw_{r,k}^m, \xi_{r,k}^m)$. For $\inner{\vz_{r,0} - \vz_{r+1,0}}{\vw^* - \vw_{r,0}}$, bringing the update rule from $\vz_{r,0}$ to $\vz_{r+1,0}$ into it yields
\begin{align*}
\inner{\vz_{r,0} - \vz_{r+1,0}}{\vw^* - \vw_{r,0}} = \frac{\eta}{M}\ssum{m}{1}{M}\ssum{k}{0}{K-1}\inner{\nabla F(\vw_{r,k}^m, \xi_{r,k}^m)}{\vw^* - \vw_{r,0}}.
\end{align*}
Note that $\EB [\nabla F (\vw_{r,k}^m, \xi_{r,k}^m)| \gF_{r,k}^m] = \nabla f_m(\vw_{r,k}^m)$, where $\gF_{r,k}^m$ is the sigma field defined as $\sigma \left(\left\{\vw_{i,j}^m;~ i = 0,\cdots, r-1,~ j = 0, \cdots, K-1 \right\}\cup \left\{ \vw_{r,j}^m;~ j = 0, \cdots, k \right\}\right)$.
Taking expectation on both sides of the above equation, we get
\begin{align}
    &\EB \inner{\vz_{r,0} - \vz_{r+1,0}}{\vw^* - \vw_{r,0}} = \frac{\eta}{M}\ssum{m}{1}{M}\ssum{k}{0}{K-1} \EB \inner{\nabla f_m(\vw_{r,k}^m)}{\vw^* - \vw_{r,0}}\\
    &\overset{(a)}{\le} \frac{\eta}{M}\ssum{m}{1}{M}\ssum{k}{0}{K-1} \EB\left\{ f_m(\vw^*) - f_m(\vw_{r,0}) + \frac{L}{2} \norm{\vw_{r,k}^m - \vw_{r,0}}_1^2 \right\}\\
    &\overset{(b)}{\le} \eta K \EB \{f(\vw^*) - f(\vw_{r,0})\} + \frac{Ld^{2/p}\eta}{2M}\ssum{m}{1}{M}\ssum{k}{0}{K-1} \EB\norm{\vw_{r,k}^m - \vw_{r,0}}_q^2. \label{eq:1_step_fedda_2}
\end{align}
Here $(a)$ holds by Lemma~\ref{lem:3_pnt_smooth} and $(b)$ holds by Lemma~\ref{lem:holder_ineq}.

On the other hand, for $\inner{\vz_{r+1,0} - \vz_{r,0}}{\vw_{r+1,0} - \vw_{r,0}}$ we have
\begin{align}
    &\EB \inner{\vz_{r+1,0} - \vz_{r,0}}{\vw_{r+1,0} - \vw_{r,0}} \overset{(a)}{\le}
    \EB \norm{\vz_{r+1,0} - \vz_{r,0}}_p^2 = \frac{\eta^2}{M^2} \EB \norm{\ssum{m}{1}{M}\ssum{k}{0}{K-1}\nabla F(\vw_{r,k}^m, \xi_{r,k}^m)}_p^2\\
    \overset{(b)}{\le}& \frac{2\eta^2}{M^2}\underbrace{\EB \norm{\ssum{m}{1}{M}\ssum{k}{0}{K-1}(\nabla F(\vw_{r,k}^m, \xi_{r,k}^m) - \nabla f_m(\vw_{r,k}^m))}_p^2}_{\gT_1} + \frac{2\eta^2}{M^2} \underbrace{\EB \norm{\ssum{m}{1}{M}\ssum{k}{0}{K-1}\nabla f_m(\vw_{r,k}^m)}_p^2}_{\gT_2}. \label{eq:1_step_fedda_2.5}
\end{align}
Here $(a)$ follows from smoothness of the conjugate of $h$ in Lemma \ref{lem:strong_cvx_mirror_map}, and $(b)$ follows from the triangle inequality and Jensen's inequality.

We bound $\gT_1$ and $\gT_2$ respectively. We abbreviate $\nabla F(\vw_{r,k}^m, \xi_{r,k}^m) - \nabla f_m(\vw_{r,k}^m)$ as $\zeta_{r,k}^m$, such that $\EB[\zeta_{r,k}^m| \gF_{r,k}^m] = 0$. Further we denote $\ssum{m}{1}{M}\zeta_{r,k}^m$ as $\zeta_{r,k}$. Then we have
\begin{align*}
\gT_1 &= \EB \left( 
\ssum{i}{1}{d}\left| \left[ \ssum{k}{0}{K-1} \zeta_{r,k} \right]_i \right|^{p}
\right)^{2/p} \overset{(a1)}{\le}
\left(
\ssum{i}{1}{d}\EB \left| \ssum{k}{0}{K-1} [\zeta_{r,k}]_i \right|^p
\right)^{2/p}\\
&\overset{(b)}{\le} \left(
C^p p^{3p/2} \ssum{i}{1}{d} \EB \left( \ssum{k}{0}{K-1} \EB [[\zeta_{r,k}]_i^2| \gF_{r,k}] \right)^{p/2}
\right)^{2/p} = Cp^3 \left(
\ssum{i}{1}{d} \EB \left( \ssum{k}{0}{K-1} \EB [[\zeta_{r,k}]_i^2| \gF_{r,k}] \right)^{p/2}
\right)^{2/p}\\
&\overset{(a2)}{\le} Cp^3 \left(
\ssum{i}{1}{d}K^{p/2} \frac{1}{K}\ssum{k}{0}{K-1} \EB\left| [\zeta_{r,k}]_i \right|^p
\right)^{2/p} = Cp^3 K\left(
\frac{1}{K}\ssum{i}{1}{d}\ssum{k}{0}{K-1} \EB \left| [\zeta_{r,k}]_i \right|^p
\right)^{2/p},
\end{align*}
where $(a1), (a2)$ hold by Jensen's inequality, $(b)$ holds by Lemma~\ref{lem:bdg_ineq}.

By making use of Lemma~\ref{lem:multi_subG} and Assumption~\ref{asp:grad_subG}, it can be seen that for 
any $i\in [d]$, $[\zeta_{r,k}]_i$ is $\sigma_M (:= \sqrt{M}\sigma)$-sub Gaussian. Then Lemma~\ref{lem:mmt_bd_subG} yields $\EB |[\zeta_{r,k}]_i|^p \le \frac{p!}{2^{p/2}(p/2)!}C^{p}M^{p/2}\sigma^p$. Plugging this into the above equation yields
\begin{align}
    \gT_1 &\le Cp^3K\left(
    \frac{1}{K}\ssum{i}{1}{d}\ssum{k}{0}{K-1}\frac{p!}{2^{p/2}(p/2)!}C^pM^{p/2}\sigma^p
    \right)^{2/p}\\
    &\le \frac{C}{2}p^3KM\sigma^2 d^{2/p}\left(\frac{p!}{(p/2)!}\right)^{2/p}
    \le Cp^4KM\sigma^2 d^{2/p}. \label{eq:1_step_fedda_t1}
\end{align}

As for the second term $\gT_2$, simply algebraic computation results in the following inequality
\begin{align*}
\gT_2 &\le 2 \EB \norm{\ssum{k}{0}{K-1}\ssum{m}{1}{M}(\nabla f_m(\vw_{r,k}^m) - \nabla f_m(\vw_{r,0}))}_p^2
+ 2 \EB \norm{KM \nabla f(\vw_{r,0})}_p^2\\
&\overset{(a)}{\le} 2 \underbrace{\EB \norm{\ssum{k}{0}{K-1}\ssum{m}{1}{M}(\nabla f_m(\vw_{r,k}^m) - \nabla f_m(\vw_{r,0}))}_p^2}_{\gT_{2,1}}
+ 4d^{2/p}K^2M^2L \EB[f(\vw_{r,0}) - f(\vw^*)].
\end{align*}
Here $(a)$ holds by Lemma~\ref{lem:holder_ineq} and Lemma~\ref{lem:conj_sc}. 
% For any vector $\vx \in \RB^d$, we can get
% \[
% \norm{\vx}_p^2 \le d^{2/p}\norm{\vx}_{\infty}^2 \text{ and }\norm{\vx}_1^2 \le d^{2/p} \norm{\vx}_q^2.
% \]
% Combining this with Assumption~\ref{asp:smooth}, then
By Assumption~\ref{asp:smooth},
\begin{align*}
\gT_{2,1} &\le \EB \left(
\ssum{k}{0}{K-1}\ssum{m}{1}{M}\norm{\nabla f_m(\vw_{r,k}^m) - \nabla f_m(\vw_{r,0})}_p
\right)^2
\le 2KM \ssum{k}{0}{K-1}\ssum{m}{1}{M} \EB \norm{\nabla f_m(\vw_{r,k}^m) - \nabla f_m(\vw_{r,0})}_p^2\\
&\le 2d^{2/p}KM\ssum{k}{0}{K-1}\ssum{m}{1}{M}\EB \norm{\nabla f_m(\vw_{r,k}^m) - \nabla f_m(\vw_{r,0})}_{\infty}^2 \le 
2d^{2/p}KML^2\ssum{k}{0}{K-1}\ssum{m}{1}{M} \EB \norm{\vw_{r,k}^m - \vw_{r,0}}_1^2\\
&\le 2d^{4/p}KML^2\ssum{k}{0}{K-1}\ssum{m}{1}{M} \EB \norm{\vw_{r,k}^m - \vw_{r,0}}_q^2.
\end{align*}
So we have
\begin{align}\label{eq:1_step_fedda_t2}
    \gT_{2} \le 4d^{4/p}KML^2\ssum{k}{0}{K-1}\ssum{m}{1}{M} \EB \norm{\vw_{r,k}^m - \vw_{r,0}}_q^2 + 4d^{2/p}K^2M^2L
    \EB [f(\vw_{r,0}) - f(\vw^*)].
\end{align}
We then obtain the bound for the inner product term $\inner{\vz_{r+1} - \vz_{r,0}}{\vw_{r+1,0} - \vw_{r,0}}$ by integrating \eqref{eq:1_step_fedda_2.5}, \eqref{eq:1_step_fedda_t1} and \eqref{eq:1_step_fedda_t2},
\begin{align}
    &\EB \inner{\vz_{r+1} - \vz_{r,0}}{\vw_{r+1,0} - \vw_{r,0}} \le
    \frac{2C\eta^2}{M^2}p^4KM\sigma^2 d^{2/p}\\
    &\quad + \frac{2\eta^2}{M^2}\left\{ 
    4d^{4/p}KML^2\ssum{k}{0}{K-1}\ssum{m}{1}{M} \EB \norm{\vw_{r,k}^m - \vw_{r,0}}_q^2
    + 4d^{2/p}K^2M^2L \EB [f(\vw_{r,0}) - f(\vw^*)]
    \right\}\\
    &= \frac{8d^{4/p} KL^2 \eta^2}{M}\ssum{k}{0}{K-1}\ssum{m}{1}{M} \EB \norm{\vw_{r,k}^m - \vw_{r,0}}_q^2 
    + 8d^{2/p}K^2L\eta^2 \EB [f(\vw_{r,0}) - f(\vw^*)]\\
    &\quad + \frac{2Cp^4d^{2/p} K \sigma^2 \eta^2}{M}. \label{eq:1_step_fedda_3}
\end{align}

Combining \eqref{eq:1_step_fedda_1}, \eqref{eq:1_step_fedda_2} and \eqref{eq:1_step_fedda_3} and applying $\norm{\vw_{r,k}^m - \vw_{r,0}}_q \leq \norm{\vz_{r,k}^m - \vz_{r,0}}_p$ from Lemma~\ref{lem:strong_cvx_mirror_map} conclude the proof of Lemma~\ref{lem:1_step_fedda}.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:local_dev_fedda}]
By Cauchy's inequality, we have
\begin{align*}
&\EB \norm{\vz_{r,k}^m - \vz_{r,0}}_p^2 = \eta^2 \EB \norm{
\ssum{i}{0}{k-1} \nabla F(\vw_{r,i}^m, \xi_{r,i}^m)
}_p^2\\
&\le 3\eta^2 \underbrace{\EB\norm{\ssum{i}{0}{k-1} (\nabla F(\vw_{r,i}^m, \xi_{r,i}^m) - \nabla f_m(\vw_{r,i}^m))}_p^2}_{\gT_1}
+ 3\eta^2 \underbrace{\EB\norm{\ssum{i}{0}{k-1}(\nabla f_m(\vw_{r,i}^m) - \nabla f_m(\vw_{r,0}))}_p^2}_{\gT_2} \\
&\quad + 3\eta^2 k^2\EB \norm{\nabla f_m(\vw_{r,0})}_p^2.
\end{align*}

Denote $\nabla F(\vw_{r,i}^m, \xi_{r,i}^m) - \nabla f_m(\vw_{r,i}^m)$ as $\zeta_{r,i}^m$. Then similar to the proof of Lemma~\ref{lem:1_step_fedda}, the following inequality can be deduced from Lemma~\ref{lem:bdg_ineq}, Jensen's inequality and Lemma~\ref{lem:mmt_bd_subG},
\begin{align*}
\gT_1 &\le Cp^3 k\left(
\frac{1}{k}\ssum{l}{1}{d}\ssum{i}{0}{k-1}\EB |[\zeta_{r,i}^m]_l|^p
\right)^{2/p}
\le Cp^3k\left( 
\frac{1}{k}\ssum{l}{1}{d}\ssum{i}{0}{k-1}\frac{p!}{2^{p/2}(p/2)!}C^p\sigma^p
\right)^{2/p}\\
&\le Cp^4 k d^{2/p}\sigma^2.
\end{align*}
The routine to bound $\gT_2$ can also be found in the proof of Lemma~\ref{lem:1_step_fedda}. Actually, we have
\begin{align*}
\gT_2 &\le \EB \left(
\ssum{i}{0}{k-1}\norm{\nabla f_m(\vw_{r,i}^m) - \nabla f_m(\vw_{r,0})}_p
\right)^2 \le k \ssum{i}{0}{k-1}\EB \norm{\nabla f_m(\vw_{r,i}^m) - \nabla f_m(\vw_{r,0})}_p^2 \\
&\overset{(a1)}{\le} k \ssum{i}{0}{k-1}d^{2/p} \EB\norm{\nabla f_m(\vw_{r,i}^m) - \nabla f_m(\vw_{r,0})}_{\infty}^2
\overset{(b)}{\le} kd^{2/p}L^2\ssum{i}{0}{k-1} \EB\norm{\vw_{r,i}^m - \vw_{r,0}}_1^2\\
&\overset{(a2)}{\le} kd^{4/p}L^2 \ssum{i}{0}{k-1} \EB \norm{\vw_{r,i}^m - \vw_{r,0}}_q^2
\overset{(c)}{\le} kd^{4/p}L^2 \ssum{i}{0}{k-1} \EB \norm{\vz_{r,i}^m - \vz_{r,0}}_p^2.
\end{align*}
Here we use Lemma~\ref{lem:holder_ineq} in $(a1), (a2)$, Assumption~\ref{asp:smooth} in $(b)$, and Lemma~\ref{lem:strong_cvx_mirror_map} in $(c)$.

Finally, using Lemma~\ref{lem:conj_sc} and Lemma~\ref{lem:holder_ineq},
\begin{align*}
\EB \norm{\nabla f_m(\vw_{r,0})}_p^2 &\le \EB \left(
\norm{\nabla f_m(\vw_{r,0}) - \nabla f_m(\vw^*)}_p + \norm{\nabla f_m(\vw^*)}_p
\right)^2\\
&\le 2\EB \norm{\nabla f_m(\vw^*)}_p^2 + 2\EB \norm{\nabla f_m(\vw_{r,0}) - \nabla f_m(\vw^*)}_p^2\\
&\le 2\EB \norm{\nabla f_m(\vw^*)}_p^2 + 2d^{2/p} \EB \norm{\nabla f_m(\vw_{r,0}) - \nabla f_m(\vw^*)}_\infty^2\\
&\le 2 \norm{\nabla f_m(\vw^*)}_p^2 + 4d^{2/p}L \EB \left\{
f_m(\vw_{r,0}) - f_m(\vw^*) - \inner{\nabla f_m(\vw^*)}{\vw_{r,0} - \vw^*}
\right\}.
\end{align*}

Combining the bounds of $\gT_1$, $\gT_2$ and $\EB \norm{\nabla f_m(\vw_{r,0})}_p^2$ yields the result of Lemma~\ref{lem:local_dev_fedda}.
\end{proof}



\begin{proof}[Proof of Lemma~\ref{lem:local_dev_scaffoldda}]
According to the update rule presented in Algorithm~\ref{alg:scaffoldda}, we have
\begin{align*}
&\EB \norm{\vz_{r,k}^m - \vz_{r,0}}_p^2 = \eta^2 \EB \norm{\ssum{i}{0}{k-1}\left[ \nabla F(\vw_{r,i}^m, \xi_{r,i}^m) - \vc_r^m + \vc_r \right]}_p^2\\
&= \eta^2 \EB \left\| \left[\ssum{i}{0}{k-1} (\nabla F(\vw_{r,i}^m, \xi_{r,i}^m)) - \nabla f_m(\vw_{r,i}^m)\right] + \left[ \ssum{i}{0}{k-1} (\nabla f_m(\vw_{r,i}^m) - \vc_{r}^m) \right]
 + k \vc_r\right\|_p^2.
\end{align*}
Note that when $\gS_r = [M]$ for all $r = 0,\cdots, R-1$, $\vc_r^m = \frac{1}{K}\ssum{k}{0}{K-1}\nabla F(\vw_{r-1,k}^m, \xi_{r-1,k}^m)$. For the sake of simplicity, we use $\zeta_{r,k}^m$, $\vartheta_{r,k}^m$ to denote $\nabla F(\vw_{r,k}^m, \xi_{r,k}^m) - \nabla f_m(\vw_{r,k}^m)$ and $\nabla f_m(\vw_{r,k}^m) - \nabla f_m(\vw_{r,0})$ respectively. Then
\begin{align*}
&\ssum{i}{0}{k-1}(\nabla f_m(\vw_{r,i}^m) - \vc_r^m)
= \ssum{i}{0}{k-1} \left\{ \vartheta_{r,i}^m + k(\nabla f_m(\vw_{r,0}) - \nabla f_m(\vw_{r-1,0})) + k(\nabla f_m(\vw_{r-1,0}) - \vc_{r}^m) \right\} \\
&= \ssum{i}{0}{k-1} \Bigg\{ \vartheta_{r,i}^m + k(\nabla f_m(\vw_{r,0}) - \nabla f_m(\vw_{r-1,0})) + \frac{k}{K}\left[K\nabla f_m(\vw_{r-1,0}) - \ssum{l}{0}{K-1}\nabla f_m(\vw_{r-1,l}^m)\right]  \\
&~~~~ + \frac{k}{K}\ssum{l}{0}{K-1}\left(\nabla f_m(\vw_{r-1,l}^m) - \nabla F(\vw_{r-1,l}^m, \xi_{r-1,l}^m)\right) \Bigg\} \\
&= \ssum{i}{0}{k-1} \left\{ \vartheta_{r,i}^m - \frac{k}{K}\ssum{l}{0}{K-1}\vartheta_{r-1,l}^m - \frac{k}{K}\ssum{l}{0}{K-1}\zeta_{r-1,l}^m +
k(\nabla f_m(\vw_{r,0}) - \nabla f_m(\vw_{r-1,0})) \right\}.
\end{align*}
Thus $\EB \norm{\vz_{r,k}^m - \vz_{r,0}}_p^2$ can be written as
\begin{align}
&\EB \norm{\vz_{r,k}^m - \vz_{r,0}}_p^2 = \eta^2 \EB
\norm{
\ssum{i}{0}{k-1}\zeta_{r,i}^m + \ssum{i}{0}{k-1}\vartheta_{r,i}^m - \frac{k}{K}\ssum{l}{0}{K-1}\zeta_{r-1,l}^m - \frac{k}{K}\ssum{l}{0}{K-1}\vartheta_{r-1,l}^m + k\vartheta_{r-1, K} + k \vc_r}_p^2\\
&\le 6\eta^2 \left\{
\EB \norm{\ssum{i}{0}{k-1}\zeta_{r,i}^m}_p^2 + \EB \norm{\ssum{l}{0}{K-1}\zeta_{r-1,l}^m}_p^2
\right\}
+ 6\eta^2 \left\{
\EB \norm{\ssum{i}{0}{k-1}\vartheta_{r,i}^m}_p^2 + \EB \norm{\ssum{l}{0}{K-1}\vartheta_{r-1,l}^m}_p^2
\right\}\\
&~~ + 6 k^2 \eta^2 \EB \norm{\vartheta_{r-1,K}^m}_p^2 + 6 k^2 \eta^2 \EB \norm{\vc_r}_p^2. \label{eq:1step_scaffolda_1}
\end{align}
Here we use $\vartheta_{r-1,K}$ to denote $\nabla f_m(\vw_{r,0}) - \nabla f_m(\vw_{r-1,0})$ with slight abuse of notation.

We start analyzing the terms appearing in the above inequality one by one. By using Lemma~\ref{lem:bdg_ineq} and Lemma~\ref{lem:mmt_bd_subG} again, for any $r \ge 0$, $k \in [K]$, the following bound can be found,
\begin{align}
    &\EB \norm{\ssum{i}{0}{k-1}\zeta_{r,i}^m}_p^2 =
    \EB \left( 
\ssum{j}{1}{d}\left| \left[ \ssum{i}{0}{k-1} \zeta_{r,i}^m \right]_j \right|^{p}
\right)^{2/p} {\le}
\left(
\ssum{j}{1}{d}\EB \left| \ssum{i}{0}{k-1} [\zeta_{r,i}^m]_j \right|^p
\right)^{2/p}\\
&{\le} \left(
C^p p^{3p/2} \ssum{j}{1}{d} \EB \left( \ssum{i}{0}{k-1} \EB [[\zeta_{r,i}^m]_j^2| \gF_{r,i}] \right)^{p/2}
\right)^{2/p} = Cp^3 \left(
\ssum{j}{1}{d} \EB \left( \ssum{i}{0}{k-1} \EB [[\zeta_{r,i}^m]_j^2| \gF_{r,i}] \right)^{p/2}
\right)^{2/p}\\
&{\le} Cp^3 \left(
\ssum{j}{1}{d}k^{p/2} \frac{1}{k}\ssum{i}{0}{k-1} \EB\left| [\zeta_{r,i}^m]_j \right|^p
\right)^{2/p} = Cp^3 k\left(
\frac{1}{k}\ssum{j}{1}{d}\ssum{i}{0}{k-1} \EB \left| [\zeta_{r,i}^m]_j \right|^p
\right)^{2/p}\\
&\le \frac{C}{2}p^3 k\sigma^2 d^{2/p}\left(\frac{p!}{(p/2)!}\right)^{2/p}
\le Cp^4 k \sigma^2 d^{2/p}. \label{eq:1step_scaffolda_2}
\end{align}
Further, it's easy to deduce that
\begin{align}
    &\EB \norm{\ssum{i}{0}{k-1}\vartheta_{r,i}^m}_p^2 \le \EB \left(
    \ssum{i}{0}{k-1}\norm{\vartheta_{r,i}^m}_p
    \right)^2 \le k \ssum{i}{0}{k-1}\EB \norm{\vartheta_{r,i}^m}_p^2\\
    \le&
    d^{2/p}k \ssum{i}{0}{k-1}\EB \norm{\nabla f_m(\vw_{r,i}^m) - \nabla f_m(\vw_{r,0})}_{\infty}^2
    \le d^{2/p}kL^2 \ssum{i}{0}{k-1}\EB \norm{\vw_{r,i}^m - \vw_{r,0}}_1^2\\
    \le&
    d^{4/p}kL^2 \ssum{i}{0}{k-1}\EB \norm{\vw_{r,i}^m - \vw_{r,0}}_q^2
    \le d^{4/p}kL^2 \ssum{i}{0}{k-1}\EB \norm{\vz_{r,i}^m - \vz_{r,0}}_p^2. \label{eq:1step_scaffolda_3}
\end{align}
For the last term, note that $\vc_r = \frac{1}{MK}\ssum{k}{0}{K-1}\ssum{m}{1}{M}\nabla F(\vw_{r-1,k}^m, \xi_{r-1,k}^m)$. Let $\zeta_{r,k} = \ssum{m}{1}{M}\zeta_{r,k}^m$, then
\begin{align}
    &\EB \norm{\vc_r}_p^2 = \EB \norm{\frac{1}{MK}\ssum{k}{0}{K-1}\ssum{m}{1}{M}\nabla F(\vw_{r-1,k}^m, \xi_{r-1,k}^m)}_p^2\\
    =& \EB \norm{\frac{1}{MK}\ssum{k}{0}{K-1}\ssum{m}{1}{M}\left\{ \zeta_{r-1,k}^m + \vartheta_{r-1,k}^m + \nabla f_m(\vw_{r-1,0}) \right\}}_p^2\\
    \le&
    \frac{3}{M^2K^2}\EB \norm{\ssum{k}{0}{K-1}\zeta_{r-1,k}}_p^2 +
    \frac{3}{M^2K^2}\EB \norm{\ssum{k}{0}{K-1}\ssum{m}{1}{M}\vartheta_{r-1,k}^m}_p^2 + 
    3\EB \norm{\nabla f(\vw_{r-1,0})}_p^2\\
    \overset{(a)}{\le}&
    \frac{Cp^4\sigma^2 d^{2/p}}{KM} + \frac{3}{MK^2}\ssum{m}{1}{M}\EB \norm{\ssum{k}{0}{K-1}\vartheta_{r-1,k}^m}_p^2 + 3\EB \norm{\nabla f(\vw_{r-1,0})}_p^2, \label{eq:1step_scaffolda_4}
\end{align}
where $(a)$ holds by making use of Lemma~\ref{lem:bdg_ineq}, \ref{lem:mmt_bd_subG} and Lemma~\ref{lem:multi_subG}. Combining \eqref{eq:1step_scaffolda_1}, \eqref{eq:1step_scaffolda_2}, \eqref{eq:1step_scaffolda_3} and \eqref{eq:1step_scaffolda_4} yields
\begin{align*}
    &\EB \norm{\vz_{r,k}^m - \vz_{r,0}}_p^2 \le C d^{4/p}kL^2\eta^2 \ssum{i}{0}{k-1}\EB \norm{\vz_{r,i}^m - \vz_{r,0}}_p^2 + 
    Cp^4\sigma^2 d^{2/p}K\left( 1  + \frac{1}{M} \right)\eta^2\\
    &+ 6\eta^2 \EB \norm{\ssum{k}{0}{K-1}\vartheta_{r-1,k}^m}_p^2 + \frac{18 \eta^2}{M}\ssum{n}{1}{M}\EB \norm{\ssum{k}{0}{K-1}\vartheta_{r-1,k}^n}_p^2 + 18 K^2\eta^2\EB \norm{\nabla f(\vw_{r-1,0})}_p^2 + 6K^2\eta^2 \EB \norm{\vartheta_{r-1,K}^m}_p^2.
\end{align*}
Summing up the above inequality with respect to the indicators $m$ and $k$ gives
\begin{align*}
    &\ssum{i}{0}{k}\ssum{m}{1}{M}\EB\norm{\vz_{r,i}^m - \vz_{r,0}}_p^2
    = \ssum{i}{0}{k-1}\ssum{m}{1}{M}\EB \norm{\vz_{r,i}^m - \vz_{r,0}}_p^2 + \ssum{m}{1}{M}\EB \norm{\vz_{r,k}^m - \vz_{r,0}}_p^2\\
    \le &
    \ssum{i}{0}{k-1}\ssum{m}{1}{M} \EB \norm{\vz_{r,i}^m - \vz_{r,0}}_p^2
    + Cd^{4/p}L^2k\eta^2 \ssum{i}{0}{k-1}\ssum{m}{1}{M} \EB \norm{\vz_{r,i}^m - \vz_{r,0}}_p^2 +
    24 \eta^2 \ssum{m}{1}{M}\EB \norm{\ssum{i}{0}{K-1}\vartheta_{r-1,i}^m}_p^2\\
    &+
    Cp^4d^{2/p}\sigma^2 MK\eta^2 + 18 MK^2\eta^2 \EB \norm{\nabla f(\vw_{r-1,0})}_p^2\\
    &+ 6K^2\eta^2\ssum{m}{1}{M}\EB \norm{\nabla f_m(\vw_{r,0}) - \nabla f_m(\vw_{r-1,0})}_p^2\\
    \overset{(a)}{\le}&
    (1 + Cd^{4/p}L^2k\eta^2)\ssum{i}{0}{k-1}\ssum{m}{1}{M}
    \EB \norm{\vz_{r,i}^m - \vz_{r,0}}_p^2 +
    24 d^{4/p}L^2K\eta^2 \ssum{i}{0}{K-1}\ssum{m}{1}{M}\EB \norm{\vw_{r-1,i}^m - \vw_{r-1,0}}_q^2\\
    +&
    Cp^4d^{2/p}\sigma^2 MK\eta^2 + 18 MK^2\eta^2 \EB \norm{\nabla f(\vw_{r-1,0})}_p^2
    + 6d^{4/p}L^2MK^2\eta^2 \EB \norm{\vw_{r,0} - \vw_{r-1,0}}_q^2.
\end{align*}
Here we use Lemma~\ref{lem:conj_sc} and Lemma~\ref{lem:holder_ineq} to deduce $(a)$.

By leveraging Lemma~\ref{lem:rcs_to_etr_fedda}, we finally get
\begin{align*}
    &\ssum{k}{0}{K-1}\ssum{m}{1}{M}\EB \norm{\vz_{r,k}^m - \vz_{r,0}}_p^2 \le 
    24 ed^{4/p}L^2K^2\eta^2 \ssum{k}{0}{K-1}\ssum{m}{1}{M}\EB \norm{\vw_{r-1,k}^m - \vw_{r-1,0}}_q^2\\
    &+
    Cd^{2/p}p^4\sigma^2 MK^2 \eta^2 + 18 eMK^3\eta^2 \EB \norm{\nabla f(\vw_{r-1,0})}_p^2\\ 
    &+ 6ed^{4/p}L^2MK^3\eta^2 \EB \norm{\vw_{r,0} - \vw_{r-1,0}}_q^2.
\end{align*}
as long as $Cd^{2/p}KL\eta \le 1$. This together with $\norm{\vw_{r,k}^m - \vw_{r,0}}_q \leq \norm{\vz_{r,k}^m - \vz_{r,0}}_p$ concludes the proof.
\end{proof}

==> theory/central_convrate.tex <==
\subsection{Convergence Rate for FedDA}
\begin{theorem}[Convergence rate for FedDA]\label{thm:conv_rt_fedda}
Suppose Assumptions~\ref{asp:convex} - \ref{asp:grad_subG} hold. Let $p=2\log d$, $\eta \le \frac{1}{48LK}$, and $\hat{\vw} := \frac{1}{R}\ssum{r}{0}{R-1}\vw_r$, where $\vw_r$ is the output of Algorithm~\ref{alg:feddualavg} in the $(r-1)$-th round. We have
\[
\EB f(\hat{\vw}) - f(\vw^*) \le \frac{4\rmD_h(\vw^*,\vw_0)}{RK\eta} +
4C(\log d)^4 \sigma^2(M^{-1} + LK\eta)\eta 
+ 216 LK^2\gE_M^*\eta^2,
\]
where $\gE_M^* := \frac{1}{M}\ssum{m}{1}{M}\norm{\nabla f_m(\vw^*)}_p^2$. Furthermore, if we take $\eta = \min \left\{ \frac{1}{48LK}, \frac{\rmD_h(\vw^*,\vw_0)^{1/3}}{(LR\gE_M^*)^{1/3}K}, \frac{\rmD_h(\vw^*,\vw_0)^{1/2}}{(RK)^{1/2}(\log d)^2 \sigma} \right\}$, then
\[
\EB f(\hat{\vw}) - f(\vw^*) \lesssim \frac{\rmD_h(\vw^*,\vw_0)L}{R} + \frac{\rmD_h(\vw^*,\vw_0)^{2/3}(L\gE_{M}^*)^{1/3}}{R^{2/3}} + \frac{\rmD_h(\vw^*,\vw_0)^{1/2}(\log d)^2 \sigma}{(RK)^{1/2}}.
\]
\end{theorem}
\subsection{Convergence Rate for ScaffoldDA}
\begin{theorem}[Convergence rate for ScaffoldDA]\label{thm:conv_rt_scaffoldda}
Suppose Assumption \ref{asp:convex} - \ref{asp:grad_subG} hold. Let $\gS_r = [M]$, $p = 2\log d$, $32d^{2/p}LK\eta \le 1$ and $\tilde{\vw} := \frac{1}{R}\ssum{r}{0}{R-1}\vw_{r,0}$. Then we have
\begin{align}
% \EB f(\tilde{\vw}) - f(\vw^*) &\le \frac{4}{RK\eta}\left\{ \EB \rmD_h(\vw^*, \vw_{r,0}) + \frac{L^2K\eta^2}{M}\gE_{r-1} + L^2K^2\eta^2\EB \norm{\vw_{0,0} - \vw_{-1,0}}_q^2 \right\}\\
% &+ \left( \frac{1}{M} + d^{4/p}LK\eta \right)Cp^4d^{2/p}\sigma^2 \eta.
\EB f(\tilde{\vw}) - f(\vw^*) &\le \frac{4\rmD_h(\vw^*, \vw_{0})}{RK\eta} + C (\log d)^4 \sigma^2 ( M^{-1} + d^{2/p}LK\eta ) \eta.
\end{align}
Furthermore, if we take $\eta = \min\left\{ \frac{1}{96LK}, \frac{\rmD_h(\vw^*,\vw_0)^{1/2}}{(RK)^{1/2}(\log d)^2 \sigma} \right\}$, then
\begin{align}
    \EB f(\tilde{\vw}) - f(\vw^*) \lesssim \frac{\rmD_h(\vw^*,\vw_0)L}{R} + \frac{\rmD_h(\vw^*,\vw_0)^{1/2}(\log d)^2 \sigma}{(RK)^{1/2}}.
\end{align}
\end{theorem}
\subsection{Proof for Main Results}
\input{Proofs/proof_for_central_conv}
